Living Scenes: Multi-object Relocalization and Reconstruction in Changing 3D Environments

Research into dynamic 3D scene understanding has primarily focused on short-term change tracking from dense observations, while little attention has been paid to long-term changes with sparse observations. We address this gap with MoRE, a novel approach for multi-object relocalization and reconstruction in evolving environments. We view these environments as "living scenes" and consider the problem of transforming scans taken at different points in time into a 3D reconstruction of the object instances, whose accuracy and completeness increase over time. At the core of our method lies an SE(3)-equivariant representation in a single encoder-decoder network, trained on synthetic data. This representation enables us to seamlessly tackle instance matching, registration, and reconstruction. We also introduce a joint optimization algorithm that facilitates the accumulation of point clouds originating from the same instance across multiple scans taken at different points in time. We validate our method on synthetic and real-world data and demonstrate state-of-the-art performance in both end-to-end performance and individual subtasks.

==> fig/tex/reg_vis.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=.8\textwidth]{fig/img/registraion_vis.pdf}
\vspace{-5px}
    \caption{\textbf{Qualitative Results of Multi-temporal Point Clouds}. From left to right: input point clouds $\times 3$, registration estimtate and ground truth.
    }
    \label{fig:reg_vis}
    % \vspace{-5px}
\end{figure*}

==> tab/3RScan_registration.tex <==
\begin{table}[t]
    \setlength{\tabcolsep}{12pt}
    \renewcommand{\arraystretch}{1.2}
	\centering
	\resizebox{\columnwidth}{!}{
   \begin{tabular}{l|cccc}
    \toprule

      Method   & \selectfont RR $\uparrow$ & MedRE $\downarrow$ &  RMSE $\downarrow$  & MedCD  $\downarrow$ \\
      \midrule
      RPMNet~\cite{yew2020rpm}& 9.40 & 3.78& 15.91 & 2.48 \\
      FreeReg~\cite{zhu2022correspondence}& 26.06 & 5.76& 11.05 & \cellcolor{tabsecond}0.82   \\
      GeoTrans.~\cite{qin2022geometric}&  \cellcolor{tabsecond}51.71 & \cellcolor{tabfirst} 3.46 & \cellcolor{tabsecond}6.51 &1.41 \\
      % \arrayrulecolor{black!10}\midrule\arrayrulecolor{black} 
      
      Ours & \cellcolor{tabfirst} 61.11 & \cellcolor{tabsecond} 3.77 & \cellcolor{tabfirst} 4.74  & \cellcolor{tabfirst}0.30 \\

    \bottomrule
    \end{tabular}
    }
    % \vspace{-3mm}
	\caption{\textbf{Results of Instance Registration on 3RScan}.}
	\label{tab:registration}
 \vspace{-1mm}
\end{table}



